Towards Empathetic Planning

Critical to successful human interaction is a capacity for empathy - the ability to understand and share the thoughts and feelings of another. As Artificial Intelligence (AI) systems are increasingly required to interact with humans in a myriad of settings, it is important to enable AI to wield empathy as a tool to benefit those it interacts with. In this paper, we work towards this goal by bringing together a number of important concepts: empathy, AI planning, and reasoning in the presence of knowledge and belief. We formalize the notion of Empathetic Planning which is informed by the beliefs and affective state of the empathizee. We appeal to an epistemic logic framework to represent the beliefs of the empathizee and propose AI planning-based computational approaches to compute empathetic solutions. We illustrate the potential benefits of our approach by conducting a study where we evaluate participants' perceptions of the agent's empathetic abilities and assistive capabilities.

==> Makefile <==
PREFIX  = main
TEXFILE = $(PREFIX).tex
PSFILE  = $(PREFIX).ps
PDFFILE = $(PREFIX).pdf

       
all:	dolatex \
	dobibtex \
	dolatex2

dolatex:
	pdflatex $(TEXFILE)

dolatex2:
	pdflatex $(TEXFILE)

dodvips:
	dvips -t letter -Ppdf -G0 -j0 -o$(PSFILE) $(PREFIX)

dopdf:
	ps2pdf $(PSFILE)

do2up:
	psnup -2 $(PSFILE) $(PREFIX)_2.ps

do4up:
	psnup -4 $(PSFILE) $(PREFIX)_4.ps

dobibtex:
	bibtex $(PREFIX)

clean:
	rm  *dvi *log *aux *bbl *blg


==> sections/empathetic_plan_recognition.tex <==
\section{Empathetic Plan Recognition}

In this section, we define the EmPR problem and its solution. We make use of work that has defined the \textit{Epistemic Plan Recognition} problem, which appeals to a notion of epistemics to (1) recognize epistemic goals (where the agent is trying to change its own (or another agent's) state of belief or knowledge, compared to an ontic goal where it is trying to change the state of the world); and (2) model the observer, and its knowledge of the actor, as first class elements of the PR process \cite{anonEPR}. We view the epistemic plan recognition paradigm in the context of empathy and formalize the notion of EmPR. In Section \ref{comp}, we describe how to integrate EmPR with EmP. Note that we assume there is only one actor. \eat{Our disucssion of EmPR in this paper is fairly brief.} We define the EmPR problem as follows:

\begin{definition}[EmPR] An empathetic plan recognition problem is a tuple $R$ $=$ $\langle Q, I, \mathcal{G}, O \rangle$, where $Q$ $= \langle \mathcal{P}, \mathcal{A}, Ag \rangle$ is an MEP domain with $\textsc{Obs}$ and $\textsc{Act}$ among the agents in $Ag$. $I \in \mathcal{L}$ is the initial KB, $\mathcal{G}$ is a set of possible goals $G \in \mathcal{L}$, and $O = o_1, ..., o_m$, is a sequence of observations. Each observation $o_j$ is a pair $(\alpha_i, \phi_i)$ comprising zero or one observed actions, $\alpha_i \in \mathcal{A}$, together with $\phi_i$, a conjunction of literals drawn from $\mathcal{P}$, or ~$\top$.
\label{EPR}
\end{definition}
% of the form $P$ $=$ $(\mathcal{P}, \mathcal{A}, Ag, I, O, \mathcal{G})$, where $I$ is the initial theory, $\mathcal{P} = \mathcal{P}_p \cup \mathcal{P}_a$ is the set of propositions (physical and affective, resp.), $\mathcal{A}$ is the set of actions, $Ag = \{E_{zer}, E_{zee}\}$ where $E_{zer}$ is empathizing with and observing $E_{zee}$, $O = [o_1, ..., o_m]$, $o_j \in \mathcal{A}$, $1$ $\leq$ $j$ $\leq$ $m$, is the sequence of observations, and $\mathcal{G}$ is the set of possible goals for the observed agent.
 

%\textbf{refelcet the new EmPR def in other papre}
Given an EmPR problem, $R$, a sequence of actions $\pi$$=$$a_1,\ldots,a_n$ {\bf satisfies} observations $O =$ $(\alpha_1, \phi_1),$$\ldots,$$(\alpha_m, \phi_m)$  if there is a monotonic function $f$ mapping the observation indices $j$ $=$ $1,...,m$ into action indices $i$ $=$ $1,...,n$ such that $a_{f(j)}$ $=$ $\alpha_j$, and $prog(I,[a_1,\ldots,a_{f(j)}]) \models\phi_j$ for $j=1,\ldots,m$. Note that since both \textsc{Obs} and \textsc{Act} are explicitly modelled in $Ag$, $I$ could encode beliefs that \text{Act} holds about \text{Obs} which can facilitate reasoning in a host of settings. E.g., if \text{Obs} believes that \text{Act} believes that \text{Obs} has already eaten dinner, then \text{Obs} can infer that \text{Act} will not wait for her to eat.

 %\textbf{change solution to reflect EPR}
 
 \begin{definition} Given an EmPR problem, $R$ $=$ $\langle Q, I, \mathcal{G}, O \rangle$, the \textbf{solution} is a plan, $\pi$, such that $\pi$ satisfies the sequence of observations, $O$, and $prog(I,\pi) \models G$ for some goal $G \in \mathcal{G}$. \label{EPR_solution}
\end{definition}

In the following sections, we use a simplified EmPR problem, where observations $o_j$ in the sequence $O$ are restricted to actions, $a \in \mathcal{A}$. $\textsc{Obs}$ is said to be \textit{maximally task-empathetic} wrt to \textsc{Act} and $R$ $=$ $\langle Q, I, \mathcal{G}, O \rangle$ and $prog(I^{\text{\textsc{ACT}}},\pi)$ progress (or are both undefined) through the same intermediate formulae for any $\pi$ that satisfies $O$ and achieves some $G \in \mathcal{G}$. This means that \textsc{Obs} needs to be empathetic `enough' to be able to generate, when taking \textsc{Act}'s perspective, all plans which \textsc{Act} can generate and that satisfy $O$ and achieve some $G \in \mathcal{G}$. Lastly, given an EmPR problem $R$ $=$ $\langle Q, I, \mathcal{G}, O \rangle$, \textsc{Obs} is maximally task-empathetic wrt to \textsc{Act} and $R$ if \textsc{Obs} empathizes with \textsc{Act}. 
% (and possibly other plans that do not meet these conditions.)



% \begin{pro}

% \end{pro}



==> sections/related_work.tex <==
\section{Related work}

%
